SESCORE2: Learning Text Generation Evaluation via Synthesizing Realistic Mistakes

Is it possible to train a general metric for evaluating text generation quality without human annotated ratings? Existing learned metrics either perform unsatisfactorily across text generation tasks or require human ratings for training on specific tasks. In this paper, we propose SESCORE2, a self-supervised approach for training a model-based metric for text generation evaluation. The key concept is to synthesize realistic model mistakes by perturbing sentences retrieved from a corpus. The primary advantage of the SESCORE2 is its ease of extension to many other languages while providing reliable severity estimation. We evaluate SESCORE2 and previous methods on four text generation tasks across three languages. SESCORE2 outperforms unsupervised metric PRISM on four text generation evaluation benchmarks, with a Kendall improvement of 0.078. Surprisingly, SESCORE2 even outperforms the supervised BLEURT and COMET on multiple text generation tasks. The code and data are available at https://github.com/xu1998hz/SEScore2.

==> 025preliminary.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/SEScore_v2_teaser.pdf}
    \caption{4-point star represents the pivot sentence. Pivot sentence: \textit{Rescaling the statement by the President of the Council.} Circles and triangles represent the sentences with minor and major mistakes, respectively. Both triangles and cycles are hard negatives. 6-point stars are easy negatives produced by the random token transformations. Circles that are inner indicates the negative samples are harder.}
    \label{fig:teaser}
\end{figure}

\paragraph{Problem Definition} 
The problem of the learned evaluation metric contains training and inference components. Ideally, given a set of reference, hypothesis, and quality score triples ($x$, $y$, $s$), we can train a supervised learned metric, $M_s: (x, y) \rightarrow s$ to predict quality score  $s*$ for unseen pair $(x*, y*)$ during inference. 

Due to the scarcity of human ratings, triples $(x,y,s)$ are unavailable for most tasks. Therefore, for the unsupervised learned metric $M_u$, it has to leverage either raw data or raw parallel data other than $(x,y,s)$ to obtain the training signals, $Q$. During inference, $M_u$, which is trained from objective $Q$, can be used to output a score $s*$ for unseen pair of $(x*, y*)$.

\paragraph{Hard Negative Construction} Constructing hard negative samples is the most essential step in the embedding learning. One common practice is to apply in-batch token insertions or replacements to the pivot sentence \cite{fu-etal-2022-contextual}. However, as shown in Figure 1, in-batch text transformations mostly produce the negative samples that are syntactically, semantically incorrect \cite{Chomsky1956ThreeMF} or both. We consider those constructed samples as easy negatives, as they largely deviate from general model mistakes \cite{Freitag_2021}. In practice, the majority of the model-generated errors can be semantically sound or syntactically correct, see triangle and circle examples in Figure \ref{fig:teaser}. Following \cite{Freitag_2021}, if the model error semantically alters the meaning of the sentence, we label them as major and minor otherwise. In both cases, they are considered as hard negatives because an ideal metric needs to capture the subtle changes between model outputs and references, in considering severity levels. This motivates us to propose a retrieval augmented data synthesis approach, which scales the diversity of synthetic texts along with the size of the raw corpus, including both major and minor error types, all three cycles in Figure \ref{fig:teaser}. 


==> 030method.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width=.98\linewidth]{fig/SEScore2_main.pdf}
%     \caption{Retrieval Augmented Data Synthesis: we denote raw pivot text, selected neighbor, and synthesized text as 4-point star, circle and triangle respectively. We randomly select a subset of proposed transformations (ticks) and estimate severity measures (SE) on them. Final score sums the individual severity measures. Final text, raw pivot text and estimated score will be used to train our quality prediction model.}
%     \label{fig:template}
% \end{figure*}

\subsection{Overview}
\method is an unsupervised learned evaluation metric initialized from the pretrained language model (e.g. BERT). From a raw text corpus, we extract text pair $(x_0, x_j)$, such that they are the k-nearest neighbor of one another. From the surface form difference of $x_0$ and $x_j$, along with the random word drops, we derive a proposal, $P$, for stratified error synthesis \cite{xu-etal-2022-not}, $P=(P_1, P_2, ..., P_n)$, such that $x_n$ can be produced through $n$ recursive text transformations from the proposed operations (eq.\ref{eq:eqn1}). 
\begin{align}
    \label{eq:eqn1}
    {\mathbf{x}}_i=\begin{cases}
    \pmb{x_0}, & \text{if } i=0 \\
    P_i(\mathbf{x}_{i-1}), & \text{0$<i\leq n$}
    \end{cases}
        %& \left\{\right .
\end{align}
We construct a severity scoring function, $S_{i}$, which takes in raw text $x_0$ and current proposal $P_i$. At each step, we estimated the severity score of the current proposal, $S_i(x_0, P_i)$. We randomly select $k$ proposals from the existing $n$ proposals. After $k$ steps, we cumulatively yield the overall quality score for the transformed text $x_k$, with the scoring label $s_k=\sum_{}^{} S_{i}(x_0, P_i)$. Please see Figure \ref{fig:template} for a concrete example. This stratified error synthesis approach can yield synthetic training triples $(x_0, x_k, s_k)$ to train our unsupervised quality prediction model. During inference, our quality prediction model can produce scores for all unseen reference and candidate pairs. Details of quality prediction model can be found in Appendix \ref{sec:quality_model}. 

\subsection{Pretraining on Synthetic Data}
The key aspect of \method is a continue pretraining technique \cite{gururangan-etal-2020-dont} that learns NLG evaluation objective during pretraining and can be inferenced directly for any text generation evaluation without fine-tuning. Ideally, the pretraining data distribution should resemble closely to the final NLG evaluation. For example, the candidate sentence outputs can come from real NLG model outputs. However, this can automatically introduce model output biases during the learning process.

To pretrain a general learned metric, we model our pretraining data construction into four constraints: 1) The pretraining data should come from a large diverse raw corpus. Therefore, \method can be generalized for different text domains and NLG tasks. 2) The synthetic data construction should be fast and independent on any text generation models. 3) The synthetic data should contain realistic and diverse model mistakes, in order to incorporate different aspects of text generation errors, such as accuracy and fluency. 4) The pretraining signals should resemble how humans grade the model outputs, namely to estimate the severity levels of each mistake \cite{Freitag_2021}. 

\subsubsection{Retrieval Augmented Data Synthesis}
Starting from a raw text sentence $x_0$, \method first map $x_0$ into the embedding space $e_0$ and find the $k$ nearest neighbors to $e_0$ through the index table search. Detailed index table construction can be found in Appendix \ref{sec:index_table}. We randomly pick one of those $k$ nearest neighbors $e_j$ and return its text form $x_j$. We use edit distance operations to model the surface form differences between $x_0$ and $x_j$. In another words, $x_0$ can go through a chain of edit operations $P$, $P = (Insert_{a\rightarrow b}, Replace_{c\rightarrow d}, Delete_{e\rightarrow f}, ...)$, where subscripts are modified text spans in sentence $x_0$, to transform into $x_j$. These edit operations, augmented with random word drops at unmodified text locations, naturally yield a set of non-overlapping insert, replace, delete operations, with respective locations to perform. Therefore, given a raw text $x_0=(t_1, ... , t_n)$ with its neighbor $x_j$ in the raw corpus, $t_i$ indicates $i$th token in $x_0$, \method can obtain proposed text transformations, $P$. To construct the synthesized text $x_k$, we randomly select a subset of $k$ text transformations from the proposal $P$ and recursively apply transformation to $x_0$. In Figure \ref{fig:template}, we demonstrate the data synthesis process from sentence pair $(x_0, x_j)$ and show an example of synthetic text $x_k$ that is constructed from the proposal. 

\subsubsection{Synthesizing Diverse Model Errors}
Synthesizing realistic and diverse hard negative pretraining data are the core challenges to learn an evaluation metric. As the recent study showed \cite{freitag-etal-2021-results}, many errors in the model outputs tend to be fluent, however, semantically deviated from the reference. To synthesize such errors, we control the text pair proximity by setting a margin criterion when retrieving the $k$ nearest neighbors \cite{schwenk-etal-2021-wikimatrix}. Based on our preliminary study, margin criterion ($k=1.06$) can retrieve sentences with similar text structure or semantics. Detailed margin criterion formulation can be found in the Appendix \ref{sec:laser_setting}. In figure \ww{Be consistent and use Figure} \ref{fig:template}, we demonstrate that our retrieval augmented data construction can synthesize errors which contextually sound but semantically deviate from the reference. To maximize the diverse error types during synthesis, we add two levels of flexibility during the proposal generation. First, all sentences $\{x_j\}$ that above the margin to the pivot sentence $x_0$ have the same probability to be selected to construct the proposal (All circles in the loop have the equal chances to be selected in Figure \ref{fig:template}). Therefore, a diverse set of lexical, syntactic and semantic dissimilarities will be considered during retrieval augmented construction. Second, we randomly select $1$ to $5$ transformations from the proposal so that synthesized text will be stratified and contain a diverse number of errors. For sentences that contain more than five errors will be labeled as the catastrophic errors with the lowest rating -25 according to the human evaluation \cite{Freitag_2021}. In Appendix \ref{sec:gen_case_study}, we demonstrate that our data synthesis pipeline can cover a diverse set of error types. One last difficulty is to synthesize positive samples of the pivot, since no ground truth is available. Inspired by \cite{gao-etal-2021-simcse}, we leverage dropout function to simulate paraphrasing embeddings by feeding the pivot twice (score: $0$). Lastly, in-batch negatives are included for the similarity lower bound (score: $-50$)\footnote{We set score $-50$ to distinguish easy and hard negatives ($-1$ to $-25$). However, $-50$ is not a sensitive hyperparamter.}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/severity_xlm.pdf}
    \caption{Source Chinese text means 'I like dogs'. Our retrieval augmented data synthesis replaces 'dog' with 'cat'. Therefore, we replace 'cat' with special token '</s>' and estimate the probability of recovering '</s>'  to 'cat' given the context of source and rest target tokens. If $p(cat|contexts) >= \gamma$, it is a minor mistake. If otherwise, it is a severe mistake. }
    \label{fig:severity_measure}
\end{figure}

\subsubsection{Pretraining Signals}
Inspired by the human grading process \cite{Freitag_2021}, we consider two levels of severity measures: major and minor, for each error in the candidate outputs. An error is major if it alters the core meaning of the sentence. To model this definition, we develop two severity measure techniques to estimate different operations separately. For insert and replace operations, we adopt a cross-lingual MLM model to perform the severity estimation, such as XLM \cite{NEURIPS2019_c04c19c2}. We first mask the perturbed locations of text $x_0$ to obtain $x_{mask, i}$ where $x_i$ is produced by a single text transformation $P_i$ on $x_0$. 
To formulate this estimation,  our severity estimation model will take in three inputs: source tokens $s=(s_0, ..., s_m)$; masked target tokens, $x_{mask,i}=(x_0, ..., x_n)$, where perturbed locations are masked; perturbed tokens $m=(m_0, ..., ,m_j)$. Then, XLM takes in concatenated source text $s$ with $x_{mask, i}$ and estimate the probability $p$ to recover span $m$ from masks. The intuition is that XLM with TLM objectives can model co-occurrences of source, target tokens and word alignments between parallel sentences. If our retrieval augmented operation $P_i$ alter the original sentence meaning, their corresponding mask location will have low probabilities to recover the perturbed tokens. By setting a threshold $\gamma$, we assign minor label to the transformation $T_i$ if $p_{mask}>=\gamma$ and severe if $p_{mask}<\gamma$. A concrete example can be found in Figure \ref{fig:severity_measure}. For delete operation, our main assumption is that delete operation creates minor error if the deleted tokens do not contain meaningful semantics in the sentence. In this case, we use token importance weight to approximate the importance of semantics that each token conveys. We adopt TF-IDF weights to estimate the importance weights. By setting a threshold $\lambda$, if the importance weights $w$ of the modified span, $w<=\lambda$, the transformation $T_i$ is minor and if $w>\lambda$, error is severe. In the end, pretraining signal for each segment is the sum of individual severity measures \footnote{$\lambda=1$ and $\gamma=0.1$ for all three languages.}.



